WeShap: Weak Supervision Source Evaluation with Shapley Values

Efficient data annotation stands as a significant bottleneck in training contemporary machine learning models. The Programmatic Weak Supervision (PWS) pipeline presents a solution by utilizing multiple weak supervision sources to automatically label data, thereby expediting the annotation process. Given the varied contributions of these weak supervision sources to the accuracy of PWS, it is imperative to employ a robust and efficient metric for their evaluation. This is crucial not only for understanding the behavior and performance of the PWS pipeline but also for facilitating corrective measures. In our study, we introduce WeShap values as an evaluation metric, which quantifies the average contribution of weak supervision sources within a proxy PWS pipeline, leveraging the theoretical underpinnings of Shapley values. We demonstrate efficient computation of WeShap values using dynamic programming, achieving quadratic computational complexity relative to the number of weak supervision sources. Our experiments demonstrate the versatility of WeShap values across various applications, including the identification of beneficial or detrimental labeling functions, refinement of the PWS pipeline, and rectification of mislabeled data. Furthermore, WeShap values aid in comprehending the behavior of the PWS pipeline and scrutinizing specific instances of mislabeled data. Although initially derived from a specific proxy PWS pipeline, we empirically demonstrate the generalizability of WeShap values to other PWS pipeline configurations. Our findings indicate a noteworthy average improvement of 5.0 points in downstream model accuracy through the revision of the PWS pipeline compared to previous state-of-the-art methods, underscoring the efficacy of WeShap values in enhancing data quality for training machine learning models.

==> 041_experiments.tex <==
\section{Experiments} \label{sec:exp}

We have undertaken comprehensive experimentation to assess the efficacy of WeShap values across a spectrum of downstream tasks. These tasks encompass identifying beneficial LFs, enhancing the PWS pipeline's accuracy, and analyzing its behaviors. Additionally, we have conducted diverse ablation studies to gauge the sensitivity of WeShap scores concerning different configuration choices.

\subsection{Setup}\label{sec:exp-setup}
\input{tables/dataset}

\paragraph{Datasets.} We evaluate our work extensively on 9 datasets, including 5 datasets for text classification (YouTube 
 \cite{alberto2015tubespam}, IMDB \cite{maas2011learning}, Yelp \cite{zhang2015character}, TREC \cite{li2002learning}, MedAbs \cite{schopf2022evaluating}), 2 datasets for tabular classification (Census \cite{misc_census_income_20}, Mushroom (MUSH) \cite{misc_mushroom_73}), and 2 datasets for image classification (Indoor-Outdoor (IND) \cite{tok2021practical}, and VOC07-Animal (VOC-A) \cite{pascal-voc-2007} \footnote{This is a binary classification version of the VOC-2007 dataset detecting whether an animal exist in the picture or not.}). {\color{blue} These datasets have been widely used to evaluate PWS pipelines in prior works \cite{zhang2021wrench,zhang2022understanding,tok2021practical, hsieh2022nemo}.}
 Table \ref{tab:dataset} outlines the dataset details and LF statistics. To assess LF quality in a scaled context, we generated LFs for the datasets using specific criteria:

For textual datasets, we employed LFs denoted as $\lambda_{k,c}$, which label class $c$ upon detecting a unigram $k$ in the text.

For tabular datasets, we utilized LFs denoted as $\lambda_{e,c}$, where class $c$ is assigned based on the truth value of expression $e$. We designed LFs for the Mushroom dataset and utilized the LF set introduced by \cite{awasthi2019learning} for the Census dataset. 

For image datasets, we employed the Azure Image Tagging API \footnote{\url{https://learn.microsoft.com/en-us/azure/ai-services/computer-vision/concept-tagging-images}} to associate tags with images corresponding to their visual features (e.g., sky, plant). Subsequently, we considered LFs denoted as $\lambda_{t,c}$, which assign class $c$ based on the existence of tag $t$.

We ensured LF quality by maintaining their accuracy at least 0.1 above random guessing on validation sets.

 \paragraph{PWS Pipeline.}
In our evaluation, we adhere to the conventional PWS pipeline framework. Initially, the label model is trained on the unlabeled training data, utilizing LFs to predict labels. Subsequently, data instances lacking active LFs are excluded from the training set. The downstream model is trained using the remaining training data, with labels predicted by the label model. To assess the holistic performance of the PWS pipeline, we measure the classification accuracy of the downstream model on the test set.

For the label model, we assess two approaches: the majority voting model and the Snorkel MeTaL model \cite{ratner2019training} implemented in WRENCH \cite{zhang2021wrench}. Regarding the downstream model, we consider two scenarios: (1) \textbf{feature extraction:} a pretrained model with frozen weights (e.g. Sentence-BERT \cite{reimers2019sentencebert}) is used to extract features from data, and the end model is trained upon the extracted features; (2) \textbf{fine-tuning:} directly fine-tune the downstream model using the weakly labeled dataset. These are the two most common adaptation methods in transfer learning \cite{peters2019tune}. For the feature extraction scenario, we employ different feature-extractors based on the dataset: Sentence-BERT \cite{reimers2019sentencebert} for YouTube, TREC, and MedAbs datasets; Bertweet-sentiment \cite{perez2021pysentimiento} for IMDB and Yelp datasets; ResNet-50 \cite{he2016deep} pretrained on ImageNet-1K \cite{deng2009imagenet} for Indoor-Outdoor and VOC07-Animal datasets. The extracted features are also used to compute KNNs for WeShap values. Then, we train a logistic regression model as the end model, which is equivalent to appending a linear layer after the pretrained models and fixing parameters in other layers. For the fine-tuning scenario, we fine-tune a pretrained BERT base model \cite{devlin2018bert} on textual datasets and a Resnet-50 model \cite{he2016deep} on image datasets.  
We set $batch\_size=32, n\_epochs=5, lr=5e-5, weight\_decay=0$ when fine-tuning BERT and $batch\_size=64, n\_epochs=50, lr=1e-4, weight\_decay=1e-5$ when fine-tuning the Resnet-50 model with an AdamW optimizer \cite{loshchilov2018decoupled} and apply early stopping technique to prevent overfitting. We do not fine-tune on tabular datasets, as they do not have corresponding pre-trained models for fine-tuning. We conduct each experiment five times with distinct seeds and report the averaged outcomes. 

 \paragraph{Baselines. } We compare the following methods. 
 \begin{description}
    \item[Random (RND):] This method assigns random values to all LFs, i.e. $V(\lambda_j)=Uniform(0,1)$. This method provides a baseline for others to compare against.

    \item[Accuracy (ACC):] This method evaluates LFs based on their accuracy on the validation set, i.e. $V(\lambda_j)=Acc(\lambda_j)$.

    \item[Coverage (COV):] This method evaluates LFs based on their coverage on the validation set, i.e. $V(\lambda_j)=Cov(\lambda_j)$.

    \item [IWS \cite{boecking2020interactive}:] This method combines the accuracy and coverage metrics to evaluate LFs, i.e. $V(\lambda_j)=(2*Acc(\lambda_j)-1)*Cov(\lambda_j)$. This corresponds to evaluating the LF based on the correct prediction count minus the wrong prediction count on the validation set.

    {\color{blue} \item [MC-Shap \cite{castro2009polynomial}:] This method utilizes Monte Carlo permutation sampling to approximate the Shapley value, using the exact label model and end model in the PWS pipeline. The total gain is evaluated based on the end model's accuracy on the validation set. To balance between approximation accuracy and runtime cost, we use $n=100$ samples in our evaluation.}

    \item[SIF \cite{zhang2022understanding}:] This method learns fine-grained source-aware influence functions, which can be aggregated to evaluate the LFs, i.e. $V(\lambda_j)=|\sum_{i,c} \bar{\phi}_{i,j,c}|$, where $\bar{\phi}_{i,j,c}$ is the source-aware influence function of $\lambda_j$ on $x_i$ with respect to class c. When computing the influence scores, we use the re-weighting method proposed in \cite{zhang2022understanding} and use the validation set as the holdout labeled dataset. 

    % \footnote{We rank the LFs based on their absolute SIF score instead of the original SIF scores; this is because we empirically find that the polarity of SIF scores tends to associate with the classes they emit. Thus, ranking the LFs based on SIF score itself, would make LFs associated with certain a class rank above the LFs for other classes and hurt downstream model performance. }

    \item[WeShap:] This is our proposed method, which utilizes Shapley values. We select the number of neighbors (K) ranging from 5 to 40. We consider Euclidean distance, Cosine distance, or Manhattan distance for distance metrics. Regarding weight functions, we choose between uniform weight (see Equation \ref{eq:weshap-instance}) and weighting by the inverse of the distance (see Equation \ref{eq:weshap-instance-weighted}). We then tailor the configuration for each dataset to optimize the accuracy of the proxy KNN classifier on the validation set.
 \end{description}
 
 \subsection{LF Evaluation}
\input{tables/lf_rank_re}

In assessing LF quality, we confront the challenge posed by the varying scales of LF evaluation metrics. To standardize this process, we implement the following methodology: initially, we arrange LFs in descending order based on their evaluation metrics, mitigating the influence of scale discrepancies. Subsequently, we adopt an iterative approach where we progressively select the top-p LFs and utilize them to train both the label and downstream models. Our evaluation commences with the top-10 LFs and incrementally expands the LF subset size at intervals of 10 until it encompasses all LFs within the dataset. We present the average accuracy of the downstream model on the test set across these iterations in Table \ref{tab:lf-rank}. 

Visualizing the number of selected LFs on the X-axis against the corresponding downstream model accuracy on the Y-axis yields a curve, and the average accuracy effectively represents the area under this curve. Theoretically, superior evaluation metrics would prioritize helpful LFs at the top, thereby enhancing downstream model accuracy across successive iterations and yielding a larger area under the accuracy curve. As this evaluation process requires training the downstream model repeatedly, which is time-consuming for the fine-tuning scenario, we only evaluated the feature-extraction scenario for the LF ranking experiments. 

As depicted in Table \ref{tab:lf-rank}, WeShap values excel in ranking beneficial LFs. Despite being derived from the proxy pipeline of MV-KNN, WeShap exhibits robust performance across various model choices. For both choices of label model, WeShap leads to the best downstream model accuracy on average, and achieves performance comparable to the best metric on all datasets except TREC, which is potentially attributable to the inferior performance of the Sentence-BERT encoder on this specific dataset, as reported in \cite{reimers2019sentencebert}. 

Particularly noteworthy is WeShap's efficacy with Snorkel being the label model, a practical PWS setting commonly employed in prior research \cite{zhang2021wrench,hsieh2022nemo,zhang2022understanding}. In this setting, WeShap improves 3.4 points over the second-best metric in average test set accuracy. In instances where WeShap surpasses competing metrics across five datasets, it boasts a substantial lead, with the most notable enhancement being a 9.5-point increase over the next best metric on the Yelp dataset. However, in scenarios where WeShap does not secure the top position, it remains a strong contender, with the performance differential between WeShap and the leading metric ranging merely from 0.9 to 1.8 points across the remaining datasets - TREC dataset being a notable exception due to the reason we explained above. 

\begin{figure}[htbp]
\centering
 \includegraphics[width=0.9\columnwidth]{figures/silhoutte_re.pdf}
 \caption{Average downstream model accuracy gain of WeShap compared to random baseline in ranking LFs.}\label{fig:acc-gain}
\end{figure}

\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/yelp-rank.png}
         % \caption{$y=x$}
         % \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/trec-rank.png}
         % \caption{$y=3\sin x$}
         % \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/voc07-rank.png}
         % \caption{$y=3\sin x$}
         % \label{fig:three sin x}
     \end{subfigure}
        \caption{Ranking LFs on selected datasets.}
        \label{fig:lf-rank-selected}
\end{figure*}


Although WeShap generally exhibits superior LF ranking performance, it occasionally produces suboptimal rankings. Thus, we focus on discerning scenarios where WeShap values reliably rank LFs. To achieve this, we analyze the data distribution across the evaluated datasets and the characteristics associated with LFs. Notably, we observe a strong correlation between WeShap's LF ranking performance and the smoothness of the training data.

The smoothness assumption, a cornerstone in semi-supervised learning, posits that points in a high-dimensional space proximal to each other should share similar labels \cite{van2020survey}. To quantify data smoothness, we employ the silhouette coefficient \cite{rousseeuw1987silhouettes}, where a higher coefficient denotes superior smoothness. Given the varying factors affecting absolute end model accuracy across datasets, we assess WeShap's efficacy by measuring its average downstream model accuracy gain relative to a random baseline. A positive gain signifies WeShap's utility in identifying beneficial LFs, while a negative gain indicates its lack of effectiveness.

Figure \ref{fig:acc-gain} depicts the silhouette coefficient plotted against the downstream model accuracy gain in the proxy framework. Evidently, a positive correlation ($r=0.810$) emerges between dataset smoothness and WeShap's accuracy gain. The rationale lies in WeShap's utilization of KNN as the downstream model within the proxy pipeline, wherein the KNN model's performance directly hinges on data smoothness. Consequently, if the dataset exhibits poor smoothness, the KNN model's accuracy diminishes, thereby impairing its efficacy as a proxy model for identifying beneficial LFs.

\subsection{PWS Pipeline Revision} \label{sec:pws-revision}
\input{tables/revision-ft}

Subsequently, we assess the impact of WeShap scores on refining the PWS pipeline regarding the downstream model's accuracy post-refinement. We explore two distinct refinement strategies: (1) Pruning: Eliminating detrimental LFs with low evaluation scores, and (2) Fine-Grained Revision: Modifying specific LF outputs or soft labels predicted by the label model.

Both WeShap and SIF support fine-grained revision, thus enabling the evaluation of both options for these methods. We designate the approaches as follows: WeShap-P (or SIF-P) for pruning out harmful LFs and WeShap-F (or SIF-F) for fine-grained revision. As for other metrics, we solely evaluate their efficacy in pruning out harmful LFs, as they lack support for fine-grained revision.

The revision pipeline operates as follows:
For LF pruning, we commence by ranking the LFs based on the evaluation metric, subsequently selecting the top-p LFs for training the label model. We tune the threshold p to optimize the PWS pipeline's accuracy on the validation dataset utilizing Optuna \cite{optuna_2019} with a Tree-structured Parzen Estimator (TPE) Sampler for 20 trials.

For fine-grained revision, we adjust threshold $\theta$ for muting LF outputs (as described in Section \ref{sec:use-cases}) for WeShap-F, and threshold $\alpha$ for perturbing train losses for SIF-F (which serves a similar purpose as $\theta$ for WeShap, as elaborated in \cite{zhang2022understanding}). We optimize these thresholds to maximize the PWS pipeline's accuracy on the validation dataset using Optuna with a TPE Sampler for 100 trials. 

Additionally, we include two baselines for comparison: the \textit{Base} method reflects the downstream model's accuracy without any revision, while the \textit{Golden} method showcases the downstream model's accuracy when trained on golden training labels without weak supervision. These baselines provide insight into the performance of specific revision methods and their disparity compared to using golden labels.

Table \ref{tab:revision} presents various revision methods' performance under feature extraction and fine-tuning scenarios. For feature extraction, we use the feature extractors described in Section \ref{sec:exp-setup} to extract fixed features from data, then train a logistic regression model for classification. For fine-tuning scenario, we fine-tune a BERT model on text datasets and a Resnet-50 model on image datasets using the revised dataset. Note that the MUSH and Census datasets are tabular ones which do not have corresponding pre-trained models for fine-tuning, so we omit the fine-tuning results on these two datasets. Due to space limitations, we report the figures when Snorkel is used as the label model. The performance comparison results are similar when using the MV model. 

We first focus on the feature-extraction scenario. In the context of LF pruning, both the WeShap-based and accuracy-based methods emerge as frontrunners, showcasing an advantage of 2.3 to 2.5 points over alternative pruning strategies. When integrating fine-grained supervision, these methodologies continue to surpass traditional LF pruning techniques. Particularly, WeShap-F distinguishes itself by outshining all other baseline methods in 7 out of 9 datasets, with the MedAbs dataset witnessing the most substantial leap in performance, an 11.7-point increase. Even in scenarios where WeShap-F doesn't claim the leading spot, such as on the YouTube and Indoor-Outdoor datasets, it remains a formidable contender, trailing the top metric by a mere 0.2-0.7 points. On average, across nine datasets, WeShap-F significantly boosts downstream model accuracy by 11.2 points over using original LFs and exceeds the performance of state-of-the-art (SOTA) revision techniques by 5.0 points. For the fine-tuning scenario, we observe similar trends, where WeShap outperforms other baseline methods in 6 out of 7 datasets and achieves competitive results in the remaining one, surpassing the performance of SOTA revision techniques by 3.9 points on average. Whether feature extraction or fine-tuning leads to better model performance is dataset-dependent, aligning with prior works' observations \cite{peters2019tune}.


% For other PWS model configurations, WeShap continues to demonstrate its excellence, outdoing all competitors in 6 to 9 out of 10 datasets, thereby achieving an average enhancement of 3.1 to 5.0 points in downstream model accuracy compared to SOTA revision techniques. 

% \input{tables/fine-tune}

% \begin{figure}[htbp]
% \centering
%  \includegraphics[width=\columnwidth]{figures/label_correction.pdf}
%  \caption{AUC score of LF evaluation metrics in correcting training label errors.}\label{fig:debug}
% \end{figure}

% Next, we explore another human-in-the-loop PWS pipeline revision method: leveraging WeShap scores to assist in identifying and manually correcting mislabeled data. We compare three distinct approaches:
% \begin{enumerate}
% \item    Sorting data points based on WeShap contribution per data point ($\sum_j w_{ij}$).
%  \item   Sorting data points using source-aware influence functions ($\sum_{j,c}\bar{\phi}_{i,j,c}$) \cite{zhang2022understanding}.
% \item    A baseline approach of randomly sorting data points.
% \end{enumerate}

% In our analysis, depicted in Figure \ref{fig:debug}, we employ Snorkel as the label model. We The resulting graph illustrates the area under the curve (AUC) when we plot the proportion of labels reviewed on X axis and the fraction of labels corrected on Y axis. Higher AUC score means the evaluation metric is better at identifying label errors. WeShap exhibits a notable proficiency in the identification of mislabeled data, leading the field with an impressive AUC improvement of up to 52.8 points over SIF in the mushroom dataset. Across ten evaluated datasets, WeShap consistently outperform baseline methods and secures an average AUC enhancement of 16.3 points over SIF, underscoring its effectiveness in label correction. 

\textbf{Weshap vs SIF.} In our examination of WeShap and SIF, both of which aim to elucidate PWS pipeline behaviors and enhance their accuracy, we delve into the specifics of these two methodologies. Both metrics are rooted in established machine learning interpretation techniques: WeShap relies on the Shapley value \cite{shapley1953value}, while SIF is grounded in the influence function \cite{koh2017understanding}, which approximates the impact of leave-one-out training. Both methods facilitate a fine-grained decomposition of influence (contribution).

In SIF, the training loss of the downstream model is dissected using the \textit{(i-j-c) effect}, quantifying the weight of the label model for $L_{ij}$ in predicting $\tilde{P}(y_i=c)$. On the other hand, WeShap is characterized by fine-grained \textit{WeShap weights} $\varphi_{ij}^c$, which gauge the \textit{average contribution} of $L_{ij}$ in predicting $\tilde{P}(y_i=c)$. This distinction underscores a key difference between these methods: while the (i-j-c) effect focuses on the weights of the current label model, the \textit{WeShap weights} considers all possible LF subsets and computes the average contribution of LFs.

To illustrate, consider the impact of $\lambda_j$ on $x_i$ concerning the MV label model. The (i-j-c) effect registers a value of 1 when $L_{ij}=c$ and 0 otherwise. However, the WeShap weight $\varphi_{ij}^c$ is also influenced by the outputs of other LFs on $x_i$, reflecting a broader perspective on LF contribution.

Another differentiating factor lies in how they adapt the Shapley value or influence function to the PWS pipeline. WeShap conceptualizes a coalition game where each LF acts as a player. Consequently, removing LFs can be directly modeled as the absence of players, while muting LF outputs can be represented as the absence of players in specific training instances. In contrast, SIF adjusts the influence function by treating each (i-j-c) effect as an individual entity and computes the influence of removing each (i-j-c) effect from training.

While this decomposition connects the influence function with PWS, it remains unclear how well the (i-j-c) effects can reflect the impact of removing specific LFs or revising weak labels. For instance, in the case of the Snorkel model with $L_{ij}=c$, altering $L_{ij}$ to $\emptyset$ does not equate to setting the (i-j-c) effect to zero. This is because the muted weak label may still exert a non-zero influence on the prediction of class c (and other classes as well). Moreover, if we retrain the label model, this change will further complicate the effects on other (i-j-c) effects.

In our evaluation, WeShap generally exhibits superior performance in ranking LFs and enhancing the accuracy of the PWS pipeline. Conclusively, although both WeShap and SIF provide insightful methodologies for decomposing the influence of LFs within the PWS pipeline, the broader and potentially more accurate reflection of LF contributions afforded by WeShap underscores its practical advantages. 


\subsection{Understanding Pipeline Behaviors}

\input{tables/lf_voc07}

We now present a case study focusing on the VOC-Animal dataset. The study aims to showcase the utilization of WeShap values in comprehending the behavior of the PWS pipeline and enhancing its performance with human-in-the-loop intervention. Class 1 indicates the presence of animals, and 0 indicates their absence. This study employs Snorkel as the label model, Resnet-50 as the feature extractor, and logistic regression as the downstream model.

Initially, the test set accuracy stood at 0.920. Table \ref{tab:lf-voc07} displays the LF statistics applied in the VOC07-Animal dataset, ranked by their respective WeShap values. Notably, the top LF assigns class 1 (indicating the presence of an animal) when the image is associated with the tag "animal," yielding a positive WeShap value of 0.024. This indicates that including this LF enhances the proxy downstream model (KNN) accuracy by an average of 0.024. Similarly, the subsequent LF, "mammal$\to$1," also exhibits a positive WeShap value of 0.015.

Given that these LFs identify tags related to specific animals, we hypothesize that incorporating LFs associated with other animals could further augment the accuracy of the PWS pipeline. Consequently, we introduce three additional LFs ("cat$\to$1," "dog$\to$1," and "bird$\to$1") into the dataset, resulting in an improved test set accuracy of 0.934.


Upon examination, we observe that the LF \textit{outdoor$\to$0} possesses a negative WeShap value of -0.022 despite achieving an accuracy of 0.66. This negative WeShap value suggests that the PWS pipeline's accuracy could likely be enhanced by eliminating this particular LF. Following removing this LF, the test set accuracy improves to 0.941.

It's worth noting that across this dataset, LFs with high WeShap values consistently exhibit very high accuracy, whereas those with low WeShap values demonstrate more modest accuracy levels ranging between 0.6 and 0.7. This observation suggests that enhancing the pipeline's accuracy may be achievable by employing a higher accuracy threshold for LF selection. Consequently, we adjusted the accuracy threshold to 0.7 and pruned out LFs with accuracies below this threshold, resulting in an improved test set accuracy of 0.957.

These revisions contributed to a total test set accuracy improvement of 0.034. This improvement should be contextualized by considering that the downstream model's accuracy using ground truth labels stands at 0.972. Therefore, achieving a 0.034 increase in downstream accuracy substantially enhances the PWS pipeline's performance.

WeShap values offer a versatile application in identifying the most influential LFs and training data pertinent to specific test instances. Illustrated in Figure \ref{fig:misprediction}, we showcase a subset of images from the validation dataset that are mispredicted by the downstream model. Subsequently, we compute WeShap scores for these mispredicted images individually.

The influential LFs are identified as those with the lowest WeShap scores, while the influential training images are determined by the images associated with the lowest WeShap contribution scores. Our analysis reveals that the mispredictions predominantly stem from certain LFs associated with the absence of animals. Consequently, users can opt to discard or downweight these LFs to rectify these mispredictions.

In cases where LFs are generally helpful but contribute negatively to specific test instances, users can execute fine-grained revision by muting the LFs specifically on the most influential training images. Additionally, it's noteworthy that certain influential LFs (e.g., \textit{tree$\to$0} in the second example) may not be active on the test instance itself. However, they can still negatively impact the test instance as they are activated on training images proximal to the test instance. WeShap values serve to pinpoint such LFs, enabling users to direct attention towards them effectively.

\begin{figure*}[htbp]
\centering
 \includegraphics[width=1.8\columnwidth]{figures/mispredictions_voc_re.pdf}
 \caption{Analyze mispredictions in VOC07-Animal dataset (Snorkel-LogReg). Class "Y" denotes presence of animals and "N" denotes absence of them. }\label{fig:misprediction}
\end{figure*}

\subsection{Ablation Studies}

\begin{figure*}[htbp]
\centering
\begin{subfigure}[c]{\columnwidth}
 \centering
 \includegraphics[width=\columnwidth]{figures/ablation_k.pdf}
 \caption{Effect of K values.}\label{fig:ablation_k}
\end{subfigure}
\hfill
\begin{subfigure}[c]{\columnwidth}
\centering
 \includegraphics[width=\columnwidth]{figures/ablation_metric.pdf}
 \caption{Effect of distance metrics.}\label{fig:ablation_distance}
\end{subfigure}

\begin{subfigure}[c]{\columnwidth}
\centering
 \includegraphics[width=\columnwidth]{figures/ablation_weight.pdf}
 \caption{Effect of weight functions.}\label{fig:ablation_weight}
\end{subfigure}
\hfill
\begin{subfigure}[c]{\columnwidth}
\centering
 \includegraphics[width=\columnwidth]{figures/ablation_valid.pdf}
 \caption{Effect of holdout dataset size.}\label{fig:ablation_valid}
\end{subfigure}
\caption{Effect of WeShap configurations for PWS pipeline revision (Snorkel-Logreg).}\label{fig:ablation}
\end{figure*}

\begin{figure}[htbp]
\centering
 \includegraphics[width=0.9\columnwidth]{figures/runtime_re.pdf}
 \caption{Runtime for different LF evaluation metrics.}\label{fig:runtime}
\end{figure}

In this section, we measure the sensitivity of WeShap scores to different configuration choices. By default, we set the number of neighbors as 10, the distance metric as Euclidean distance, and the weight function as uniform weight. We evaluate the performance of WeShap score using the downstream model accuracy after fine-grained PWS pipeline revision (WeShap-F) and evaluate the following configuration choices:
\begin{description}
\item[Number of Neighbors (K): ]We evaluate four choices of K: 5, 10, 20, and 40 when calculating WeShap values.

\item[Distance Metrics: ]We test three distance metrics for calculating nearest neighbors: Cosine distance, Euclidean distance, and Manhattan distance. 

\item[Weight Functions: ]We evaluate two options for averaging the contribution of neighbor points when calculating WeShap scores: uniform weight (Equation \ref{eq:weshap-instance}) and weight by the inverse of distance (Equation \ref{eq:weshap-instance-weighted}).

\item[Holdout Dataset Size:] We change the holdout dataset size by randomly sampling from the original validation dataset for calculating the WeShap scores. As the evaluated datasets have diverse validation dataset sizes, we pick 6 datasets where the original validation dataset contains over 800 points and evaluate 5 choices of the holdout dataset size: 50, 100, 200, 400, and 800. 

\end{description}

The findings, as depicted in Figure \ref{fig:ablation}, demonstrate the robustness of WeShap scores in enhancing the PWS pipeline, irrespective of variations in K values, distance metrics, and weight functions. Moreover, enlarging the holdout dataset consistently enhances the performance of the PWS pipeline. Specifically, doubling the holdout dataset size correlates with a 1.2-point increase in downstream model accuracy across our experiments. Remarkably, even with as few as 50 labeled data points, WeShap scores contribute to a substantial 5.7-point average improvement in downstream model accuracy compared to the original PWS pipeline. These results underscore the continued utility of WeShap scores, particularly in scenarios with constrained labeling budgets.

\subsection{Runtime}

The runtime experiments were executed on a computing platform featuring a 4-core Intel(R) Xeon(R) Gold 5122 CPU with a base frequency of 3.60 GHz and an NVIDIA TITAN Xp GPU boasting 12 GB of memory. The GPU was exclusively utilized to compute the SIF score. The runtime results are presented in Figure \ref{fig:runtime}. Specifically, the reported runtimes pertain to the computation of LF evaluation metrics, excluding the time required to train the label model or the end model, thus focusing solely on the computational cost associated with the metrics themselves. The experiments were repeated 5 times, and the average runtime is reported alongside error bars indicating the standard deviation.

Figure \ref{fig:runtime} showcases that WeShap scores can be computed within seconds across the evaluated datasets. Conversely, even when leveraging GPU acceleration, SIF necessitates significantly more time than other methods. This discrepancy arises because SIF involves the computation of Hessian-vector products through a recursive procedure, which incurs substantial computational overhead. Consequently, WeShap enjoys a distinct advantage in terms of efficient and lightweight LF evaluation.
